Rethinking the Form of Latent States in Image Captioning

RNNs and their variants have been widely adopted for image captioning. In RNNs, the production of a caption is driven by a sequence of latent states. Existing captioning models usually represent latent states as vectors, taking this practice for granted. We rethink this choice and study an alternative formulation, namely using two-dimensional maps to encode latent states. This is motivated by the curiosity about a question: how the spatial structures in the latent states affect the resultant captions? Our study on MSCOCO and Flickr30k leads to two significant observations. First, the formulation with 2D states is generally more effective in captioning, consistently achieving higher performance with comparable parameter sizes. Second, 2D states preserve spatial locality. Taking advantage of this, we visually reveal the internal dynamics in the process of caption generation, as well as the connections between input visual domain and output linguistic domain.

==> exprt.tex <==
% !TEX root = main.tex

\section{Experiments}
\label{sec:exprt}

We report our experiments on MSCOCO~\cite{lin2014microsoft} and Flickr30k~\cite{young2014image}, 
which compare the proposed formulation with the standard one, 
and also present studies that 
interpret the latent states of the learned models.

\subsection{Experiment Settings}

MSCOCO~\cite{lin2014microsoft} contains $123,287$ images.
We follow the splits in \cite{karpathy2015deep},
using $112,585$ images for training, $5,000$ for validation, and the
remaining $5,000$ for testing.
Flickr30K~\cite{young2014image}~contains $31,783$ images in total,
and we follow splits in \cite{karpathy2015deep},
which has $1,000$ respectively for validation and testing,
and the rest for training.
%
In both datasets, each image comes with $5$ ground-truth captions.
To obtain a vocabulary, we turn words to lowercase and remove those with non-alphabet characters
Then, we replaced the words
that appear less than $5$ times with a special token \emph{UNK},
resulting in a vocabulary of size $9,487$ for MSCOCO, and $7,000$ for Flickr30k. 
Following the common convention~\cite{karpathy2015deep}, we truncated all ground-truth
captions to have at most $16$ words.

All captioning methods in our experiments are based on the encoder-decoder
paradigm~\cite{vinyals2015show}. We use
ResNet-152~\cite{He2015} pretrained on ImageNet \cite{ILSVRC15} as the encoder
in all methods.
In particular, we take the output of the layer \texttt{res5c} as
the visual features $\mV$.
We refer to different types of decoders as the combination of cell type and state shape.
\eg~\emph{LSTM-1DS-($L$)} refers to a standard LSTM-based decoder with latent states of size $L$,
and \emph{GRU-2DS-($C,H,W$)} refers to an RNN-2DS decoder with GRU cells as
in Eq.\eqref{eq:gru_update}, whose latent states are of size $C \times H \times W$.
%
Moreover, all RNN-2DS models adopt a raw word-embedding of size
$4 \times 15 \times 15$, except when a different size is explicitly specified.
The convolution kernels $\mK_h$, $\mK_x$, and $\mK_v$ share the same size
$C \times C \times 3 \times 3$. 

The focus of this paper is the representations of latent states.
To ensure a fair comparison, 
no additional modules including the attention module \cite{xu2015show}~are added to all methods.
Moreover, no other training strategies are utilized, such as the scheduled sampling \cite{bengio2015scheduled},
except for the maximum likelihood objective,
where we use SGD with the ADAM optimizer~\cite{kingma2014adam}.
During training, we first fix the CNN encoder and optimize the decoder
with learning rate $0.0004$ in the first $20$ epochs, and then
jointly optimize both the encoder and decoder with learning rate $0.00001$,
until performances on the validation set saturate.

As for evaluation, we report results using metrics including 
BLEU-4 (B4)~\cite{papineni2002bleu}, METEOR (MT)~\cite{lavie2014meteor},
ROUGE (RG)~\cite{lin2004rouge}, CIDER (CD)~\cite{vedantam2015cider},
and SPICE (SP)~\cite{anderson2016spice}.

\subsection{Comparative Analysis}

\input{fig_lstm1ds_rnn2ds.tex}

First, we compared \emph{RNN-2DS} with \emph{LSTM-1DS},
for the former has 2D states with the simplest type of cells
while the latter has 1D states with sophisticated LSTM cells. 
As the capacity of a model is closely related to the number of parameters,
to ensure a fair comparison, each config of \emph{RNN-2DS} is compared to
an \emph{LSTM-1DS} config \emph{with a similar number of parameters}.
In this way, the comparative results will signify the differences in
the inherent expressive power of both formulations.

The resulting curves in terms of different metrics are listed in Figure \ref{fig:curve_1dvs2d},
in which we can see that
\emph{RNN-2DS} outperforms
\emph{LSTM-1DS} consistently,
across different parameter sizes and under different metrics.
%
These results show that \emph{RNN-2DS}, with the states that preserve
spatial locality, can capture both visual and linguistic information
more efficiently.

\input{tab_rnn2ds_cell.tex}

We also compared different types of decoders with similar number of parameters,
namely \emph{RNN-1DS}, \emph{GRU-1DS}, \emph{LSTM-1DS}, \emph{RNN-2DS}, and \emph{GRU-2DS}.
Table \ref{tab:rnn2ds_cell} shows the results of these decoders on both datasets, 
from which we observe:
%
(1) \emph{RNN-2DS} outperforms \emph{RNN-1DS}, \emph{GRU-1DS}, and \emph{LSTM-1DS}, 
indicating embedding latent states in 2D forms is more effective.
(2) \emph{GRU-2DS}, which is also based on the proposed formulation but add several gate functions, 
surpasses other decoders and
yields the best result. 
This suggests that
the techniques developed for conventional RNNs including gate functions
and attention modules~\cite{xu2015show} are very likely to benefit RNNs
with 2D states as well.

\input{tab_designchoice.tex}

Table \ref{tab:designchoice} also compares the performances obtained with
different design choices in \emph{RNN-2DS},
including pooling methods, activation functions, and sizes of word embeddings, kernels and latent states
The results show that mean pooling outperforms
max pooling by a significant margin, indicating that information from all
locations is significant.
The best combination for \emph{RNN-2DS} with $256$ channels uses mean pooling and ReLU, as well as word embeddings, kernels and latent states of sizes respectively 
$1\times15\times15$, $3\times$ and $256\times7\times7$.

Figure \ref{fig:qualitative} includes some qualitative samples,
in which we can see
the captions generated by \emph{LSTM-1DS} rely heavily on the language priors,
which sometimes contain the phrases that are not consistent with the visual
content but appear frequently in training captions.
On the contrary, the sentences from \emph{RNN-2DS} and \emph{GRU-2DS}
are more relevant to the visual content.

\input{fig_qualitative.tex}

\input{fig_wordchannel.tex}
\input{fig_seqchannel.tex}

\subsection{Visual Study for RNN-2DS}

A key benefit of \emph{RNN-2DS} is the improved interpretability.
Specifically, \emph{RNN-2DS} allows us to visualize the channels using the methods
introduced in section \ref{sub:actreg} and section \ref{sub:wordchannel}.
In this study, we used \emph{RNN-2DS-($512, 7, 7$)},
as it contains a large number of channels for analysis.
%
Specifically, we identified the channels associated with different words
using the \emph{association score} defined in Eq.\eqref{eq:vis_cor}
and then visualized these channels by finding the \emph{activated region}
(see Sec.~\ref{sub:actreg}).
%
Figure~\ref{fig:wordchannel} visualizes several latent channels,
showing the activated regions on those images that contain their
associated words in the corresponding generated captions.

Besides the visual samples in Figure \ref{fig:wordchannel}, we also
had some empirical findings:
(1) Only nouns have strong associations with channels, which is
consistent with the fact that spatial locality is highly-related with
the visual entities described as nouns.
(2) Some channels have multiple associated nouns. For example,
\emph{Channel}-$066$ is associated with
\emph{``cat''}, \emph{``dog''}, and \emph{``cow''}.
This is not surprising -- since there are more nouns in the vocabulary than
the number of channels, some nouns have to share channels.
Here, it is worth noting that the nouns that share a channel tend to be
visually relevant. This shows that the latent channels
can capture meaningful visual structures.
(3) The activated regions of channels often capture the visual entities
corresponding to the associated nouns, but they may also reflect the
surrounding context occasionally.
(4) Not all channels have associated words. Some channels may capture
abstract notions instead of visual elements. The interpretation of such
channels is an interesting direction in future.

As shown in Figure \ref{fig:seqchannel}, the activated regions not only help to visualize a channel, but also
reflect the \emph{dynamics} of the decoding process.
Specifically, for a noun, we found that the activated regions of
its associated channel become significant as the decoding process approaches
the point where the noun is produced, and the channel becomes deactivated
afterwards.
Intuitively, this indicates that the channel is only activated to provide
visual cues when it is needed, \eg~at the decoding steps where this noun is
close to being generated. This is consistent with our assumption in
section~\ref{sub:wordchannel}.

